A parameter scan of dark zone maintenance for high-contrast imaging of exoplanets using theoretical and experimental implementations

Maintaining wavefront stability while directly imaging exoplanets over long exposure times is an ongoing problem in the field of high-contrast imaging. Robust and efficient high-order wavefront sensing and control systems are required for maintaining wavefront stability to counteract mechanical and thermal instabilities. Dark zone maintenance (DZM) has been proposed to address quasi-static optical aberrations and maintain high levels of contrast for coronagraphic space telescopes. To further experimentally test this approach for future missions, such as the Habitable Worlds Observatory, this paper quantifies the differences between the theoretical closed-loop contrast bounds and DZM performance on the High-contrast Imager for Complex Aperture Telescopes(HiCAT) testbed. The quantification of DZM is achieved by traversing important parameters of the system, specifically the total direct photon rate entering the aperture of the instrument, ranging from $1.85 \times 10^6$ to $1.85 \times 10^8$ photons per second, and the wavefront error drift rate, ranging from $\sigma_{drift}$ = 0.3 - 3 $nm/\sqrt{iteration}$, injected via the deformable mirror actuators. This is tested on the HiCAT testbed by injecting random walk drifts using two Boston Micromachines kilo deformable mirrors (DMs). The parameter scan is run on the HiCAT simulator and the HiCAT testbed where the corresponding results are compared to the model-based theoretical contrast bounds to analyze discrepancies. The results indicate an approximate one and a half order of magnitude difference between the theoretical bounds and testbed results.

==> bib_location.tex <==
https://zbib.org/d607c139920248f097df19445bdc00ef
